Word Alignment as Preference for Machine Translation

The problem of hallucination and omission, a long-standing problem in machine translation (MT), is more pronounced when a large language model (LLM) is used in MT because an LLM itself is susceptible to these phenomena. In this work, we mitigate the problem in an LLM-based MT model by guiding it to better word alignment. We first study the correlation between word alignment and the phenomena of hallucination and omission in MT. Then we propose to utilize word alignment as preference to optimize the LLM-based MT model. The preference data are constructed by selecting chosen and rejected translations from multiple MT tools. Subsequently, direct preference optimization is used to optimize the LLM-based model towards the preference signal. Given the absence of evaluators specifically designed for hallucination and omission in MT, we further propose selecting hard instances and utilizing GPT-4 to directly evaluate the performance of the models in mitigating these issues. We verify the rationality of these designed evaluation methods by experiments, followed by extensive results demonstrating the effectiveness of word alignment-based preference optimization to mitigate hallucination and omission. On the other hand, although it shows promise in mitigating hallucination and omission, the overall performance of MT in different language directions remains mixed, with slight increases in BLEU and decreases in COMET.

==> figures/ablation_comet.tex <==
\begin{figure}[ht!]
    \centering
    % \resizebox{\columnwidth}{!}{
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figures/ablation_hard_comet.pdf}
        \caption{Hard instances}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \includegraphics[width=\textwidth]{figures/ablation_easy_comet.pdf}
        \caption{Easy instances}
    \end{subfigure}
    \caption{Ablation study. Results in COMET is demonstrated. Higher COMET is better. For fair comparison the range of y-axis are the same for hard instances and easy instances. Refer to \S\ref{sec:ablation} for discussion.
    }
    \label{fig:ablation_comet}
\end{figure}

==> figures/gpt_eval_result.tex <==
\begin{figure*}[ht]
% \small
    \centering
% \resizebox{1.5\textwidth}{!}{
    
    \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/gpt_eval_n_100.pdf}
         \caption{n=100}
         \label{fig:gpt_eval_n_100}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/gpt_eval_n_200.pdf}
         \caption{n=200}
         \label{fig:gpt_eval_n_200}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.3\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/gpt_eval_n_500.pdf}
         \caption{n=500}
         \label{fig:gpt_eval_n_500}
     \end{subfigure}
     % \hfill
     % \begin{subfigure}{0.24\textwidth}
     %     \centering
     %      \includegraphics[width=\linewidth]{figures/comet_good.pdf}
     %     \caption{}
     %     \label{fig:comet_good}
     % \end{subfigure}
     
    % }
    \caption{\qy{the meaning of y-axis}}
    \label{fig:gpt_eval_results}
\normalsize
\end{figure*}

==> figures/subset_result.tex <==
\begin{figure*}[ht]
\small
    \centering
% \resizebox{1.5\textwidth}{!}{
    
    \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bleu_bad_n=100.pdf}
         \caption{BLEU on hard instances.}
         \label{fig:bleu_bad_100}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/bleu_good_n=100.pdf}
         \caption{BLEU on easy instances.}
         \label{fig:bleu_good_100}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/comet_bad_n=100.pdf}
         \caption{COMET on hard instances.}
         \label{fig:comet_bad_100}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/comet_good_n=100.pdf}
         \caption{COMET on easy instances.}
         \label{fig:comet_good_100}
     \end{subfigure}
     
    % }
    \caption{Comparison of \methodname{} and baseline when $N=100$.}
    \label{fig:subset_res_100}
\normalsize
\end{figure*}

\begin{figure*}[ht]
\small
    \centering
% \resizebox{1.5\textwidth}{!}{
    
    \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bleu_bad_n=200.pdf}
         \caption{BLEU on hard instances.}
         \label{fig:bleu_bad_200}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/bleu_good_n=200.pdf}
         \caption{BLEU on easy instances.}
         \label{fig:bleu_good_200}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/comet_bad_n=200.pdf}
         \caption{COMET on hard instances.}
         \label{fig:comet_bad_200}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/comet_good_n=200.pdf}
         \caption{COMET on easy instances.}
         \label{fig:comet_good_200}
     \end{subfigure}
     
    % }
    \caption{Comparison of \methodname{} and baseline when $N=200$.}
    \label{fig:subset_res_200}
\normalsize
\end{figure*}

\begin{figure*}[ht]
\small
    \centering
% \resizebox{1.5\textwidth}{!}{
    
    \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/bleu_bad_n=500.pdf}
         \caption{BLEU on hard instances.}
         \label{fig:bleu_bad_500}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/bleu_good_n=500.pdf}
         \caption{BLEU on easy instances.}
         \label{fig:bleu_good_500}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figures/comet_bad_n=500.pdf}
         \caption{COMET on hard instances.}
         \label{fig:comet_bad_500}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
         \centering
          \includegraphics[width=\linewidth]{figures/comet_good_n=500.pdf}
         \caption{COMET on easy instances.}
         \label{fig:comet_good_500}
     \end{subfigure}
     
    % }
    \caption{Comparison of \methodname{} and baseline when $N=500$.}
    \label{fig:subset_res_500}
\normalsize
\end{figure*}

==> tables/all_results_bak.tex <==
\begin{table}[]
\begin{tabular}{c|c|cc}
\hline
Test Set               & Method   & BLEU  & COMET \\ \hline
\multirow{2}{*}{De-En} & Alma 13B & 30.73 & 84.42 \\
                       & Ours     & 31.93 & 84.51 \\ \hline
\multirow{2}{*}{Cs-En} & Alma 13B & 44.68 & 86.29 \\
                       & Ours     & 45.60 & 86.53 \\ \hline
\multirow{2}{*}{Is-En} & Alma 13B & 36.46 & 86.30 \\
                       & Ours     & 38.85 & 86.45 \\ \hline
\multirow{2}{*}{Zh-En} & Alma 13B & 24.65 & 79.90 \\
                       & Ours     & 23.94 & 80.05 \\ \hline
\multirow{2}{*}{Ru-En} & Alma 13B & 40.37 & 85.09 \\
                       & Ours     & 40.09 & 85.23 \\ \hline
\multirow{2}{*}{Avg}   & Alma 13B & 35.37 & 84.40 \\
                       & Ours     & 36.08 & 84.55 \\ \hline
\end{tabular}
\end{table}

==> tables/all_results_noavg.tex <==
\begin{table*}[]
\caption{Specific results on 10 translation directions. The size of models are 13B. BLEU and COMET are reported. Cells where the difference is larger than $1.0$ are highlighted with colored background. \textcolor{cyan}{Blue} indicates ours model outperforms ALMA and \textcolor{red}{red} indicates the opposite.}
\label{tab:all_results}
% \resizebox{\textwidth}{!}{
\centering
\begin{tabular}{ccccccccccc}
\hline
Model-\scriptsize{Metric} & de-en & cs-en & is-en & zh-en & ru-en & en-de & en-cs & en-is & en-zh & en-ru \\
\hline
\multicolumn{11}{c}{\textit{N=100}} \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Easy instances}} \\
ALMA-\scriptsize{BLEU} & \cellcolor{cyan!50}31.38 & 45.79 & \cellcolor{cyan!50}38.14 & 25.64 & 41.25 & 32.09 & 31.95 & \cellcolor{red!50}27.57 & 40.05 & 29.37 \\
Ours-\scriptsize{BLEU} & \cellcolor{cyan!50}32.50 & 46.32 & \cellcolor{cyan!50}40.13 & 25.23 & 40.80 & 31.22 & 31.55 & \cellcolor{red!50}26.00 & 39.55 & 29.01 \\
ALMA-\scriptsize{COMET} & 85.57 & 87.71 & 87.82 & 81.38 & 86.26 & 86.84 & \cellcolor{red!50}90.90 & \cellcolor{red!50}87.61 & 87.14 & 88.80 \\
Ours-\scriptsize{COMET} & 85.50 & 87.67 & 87.71 & 81.24 & 86.17 & 86.02 & \cellcolor{red!50}89.84 & \cellcolor{red!50}85.80 & 86.39 & 87.89 \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Hard instances}} \\
ALMA-\scriptsize{BLEU} & \cellcolor{cyan!50}12.25 & \cellcolor{cyan!50}29.49 & \cellcolor{cyan!50}21.72 & \cellcolor{cyan!50}1.95 & \cellcolor{cyan!50}15.73 & 15.71 & \cellcolor{cyan!50}12.79 & 17.51 & \cellcolor{cyan!50}14.59 & 15.45 \\
Ours-\scriptsize{BLEU} & \cellcolor{cyan!50}15.56 & \cellcolor{cyan!50}35.93 & \cellcolor{cyan!50}27.72 & \cellcolor{cyan!50}4.62 & \cellcolor{cyan!50}19.77 & 16.15 & \cellcolor{cyan!50}16.67 & 17.13 & \cellcolor{cyan!50}19.49 & 15.54 \\
ALMA-\scriptsize{COMET} & \cellcolor{cyan!50}62.73 & \cellcolor{cyan!50}67.08 & \cellcolor{cyan!50}72.62 & \cellcolor{cyan!50}49.94 & \cellcolor{cyan!50}62.64 & \cellcolor{cyan!50}58.50 & \cellcolor{cyan!50}60.80 & \cellcolor{cyan!50}70.02 & \cellcolor{cyan!50}59.07 & \cellcolor{cyan!50}62.31 \\
Ours-\scriptsize{COMET} & \cellcolor{cyan!50}65.98 & \cellcolor{cyan!50}71.16 & \cellcolor{cyan!50}75.12 & \cellcolor{cyan!50}58.99 & \cellcolor{cyan!50}67.19 & \cellcolor{cyan!50}60.90 & \cellcolor{cyan!50}67.90 & \cellcolor{cyan!50}71.57 & \cellcolor{cyan!50}62.03 & \cellcolor{cyan!50}65.16 \\
\hline
\multicolumn{11}{c}{\textit{N=200}} \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Easy instances}} \\
ALMA-\scriptsize{BLEU} & \cellcolor{cyan!50}31.96 & 47.11 & 39.94 & 26.22 & 42.13 & 32.50 & 32.75 & \cellcolor{red!50}28.54 & 41.08 & 30.22 \\
Ours-\scriptsize{BLEU} & \cellcolor{cyan!50}33.10 & 47.41 & 41.60 & 25.79 & 41.43 & 31.52 & 32.20 & \cellcolor{red!50}26.91 & 40.48 & 29.79 \\
ALMA-\scriptsize{COMET} & 86.34 & 88.61 & 88.72 & 82.31 & 87.02 & \cellcolor{red!50}87.76 & \cellcolor{red!50}91.85 & \cellcolor{red!50}88.67 & 87.97 & 89.67 \\
Ours-\scriptsize{COMET} & 86.16 & 88.40 & 88.43 & 81.98 & 86.89 & \cellcolor{red!50}86.75 & \cellcolor{red!50}90.77 & \cellcolor{red!50}86.94 & 87.12 & 88.73 \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Hard instances}} \\
ALMA-\scriptsize{BLEU} & \cellcolor{cyan!50}17.46 & \cellcolor{cyan!50}30.39 & \cellcolor{cyan!50}24.17 & \cellcolor{cyan!50}6.00 & \cellcolor{cyan!50}20.03 & 19.11 & \cellcolor{cyan!50}14.83 & 19.02 & \cellcolor{cyan!50}18.61 & 15.43 \\
Ours-\scriptsize{BLEU} & \cellcolor{cyan!50}19.31 & \cellcolor{cyan!50}35.04 & \cellcolor{cyan!50}29.25 & \cellcolor{cyan!50}7.55 & \cellcolor{cyan!50}23.70 & 19.96 & \cellcolor{cyan!50}18.16 & 18.29 & \cellcolor{cyan!50}21.52 & 15.95 \\
ALMA-\scriptsize{COMET} & \cellcolor{cyan!50}67.24 & \cellcolor{cyan!50}71.82 & \cellcolor{cyan!50}76.62 & \cellcolor{cyan!50}57.84 & \cellcolor{cyan!50}67.59 & \cellcolor{cyan!50}64.30 & \cellcolor{cyan!50}67.13 & 74.56 & 65.46 & \cellcolor{cyan!50}67.59 \\
Ours-\scriptsize{COMET} & \cellcolor{cyan!50}69.85 & \cellcolor{cyan!50}74.82 & \cellcolor{cyan!50}78.52 & \cellcolor{cyan!50}63.87 & \cellcolor{cyan!50}70.22 & \cellcolor{cyan!50}66.77 & \cellcolor{cyan!50}70.37 & 74.13 & 67.50 & \cellcolor{cyan!50}68.78 \\
\hline
\multicolumn{11}{c}{\textit{N=500}} \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Easy instances}} \\
ALMA-\scriptsize{BLEU} & 34.36 & 50.81 & 46.92 & 28.50 & 45.16 & \cellcolor{red!50}34.61 & \cellcolor{red!50}35.28 & \cellcolor{red!50}31.79 & 43.91 & 32.13 \\
Ours-\scriptsize{BLEU} & 35.33 & 50.59 & 47.25 & 27.82 & 44.16 & \cellcolor{red!50}33.25 & \cellcolor{red!50}34.07 & \cellcolor{red!50}30.00 & 42.92 & 31.67 \\
ALMA-\scriptsize{COMET} & 88.08 & 90.54 & 91.04 & 84.29 & 88.62 & \cellcolor{red!50}89.59 & \cellcolor{red!50}93.66 & 91.08 & 89.79 & 91.47 \\
Ours-\scriptsize{COMET} & 87.80 & 90.10 & 90.50 & 83.86 & 88.40 & \cellcolor{red!50}88.55 & \cellcolor{red!50}92.48 & 89.57 & 88.79 & 90.61 \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Hard instances}} \\
ALMA-\scriptsize{BLEU} & \cellcolor{cyan!50}21.31 & \cellcolor{cyan!50}35.46 & \cellcolor{cyan!50}28.66 & 13.08 & \cellcolor{cyan!50}25.4 & 22.53 & \cellcolor{cyan!50}19.82 & \cellcolor{red!50}22.52 & \cellcolor{cyan!50}24.81 & 19.78 \\
Ours-\scriptsize{BLEU} & \cellcolor{cyan!50}23.09 & \cellcolor{cyan!50}37.91 & \cellcolor{cyan!50}32.66 & 14.04 & \cellcolor{cyan!50}27.32 & 22.89 & \cellcolor{cyan!50}22.38 & \cellcolor{red!50}21.32 & \cellcolor{cyan!50}26.58 & 19.78 \\
ALMA-\scriptsize{COMET} & \cellcolor{cyan!50}73.56 & \cellcolor{cyan!50}78.24 & 81.55 & \cellcolor{cyan!50}67.07 & \cellcolor{cyan!50}74.39 & 72.74 & 76.38 & \cellcolor{red!50}80.61 & 73.38 & 75.29 \\
Ours-\scriptsize{COMET} & \cellcolor{cyan!50}74.77 & \cellcolor{cyan!50}79.75 & 82.41 & \cellcolor{cyan!50}69.56 & \cellcolor{cyan!50}75.63 & 73.24 & 77.34 & \cellcolor{red!50}79.19 & 74.12 & 74.97 \\
\hline
\multicolumn{11}{c}{\textit{Overall performance, i.e., N=infinite when all instances are included.}} \\
ALMA-\scriptsize{BLEU} & \cellcolor{cyan!50}30.73 & 44.68 & \cellcolor{cyan!50}36.46 & 24.15 & 40.37 & 31.37 & 31.12 & \cellcolor{red!50}26.67 & 39.05 & 28.76 \\
Ours-\scriptsize{BLEU} & \cellcolor{cyan!50}31.93 & 45.60 & \cellcolor{cyan!50}38.85 & 23.94 & 40.09 & 30.64 & 30.91 & \cellcolor{red!50}25.22 & 38.76 & 28.43 \\
ALMA-\scriptsize{COMET} & 84.42 & 86.29 & 86.30 & 79.70 & 85.09 & 85.45 & 89.42 & \cellcolor{red!50}85.85 & 85.76 & 87.50 \\
Ours-\scriptsize{COMET} & 84.50 & 86.53 & 86.45 & 80.05 & 85.22 & 84.78 & 88.75 & \cellcolor{red!50}84.38 & 85.19 & 86.77 \\
\hline
\end{tabular}
% }
\end{table*}

==> tables/all_results_nocolor.tex <==
\begin{table*}[]
\caption{Specific results on 10 translation directions. The size of models are 13B. BLEU and COMET are reported.}
\label{tab:all_results}
% \resizebox{\textwidth}{!}{
\centering
\begin{tabular}{ccccccccccc}
\hline
Model-\scriptsize{Metric} & de-en & cs-en & is-en & zh-en & ru-en & en-de & en-cs & en-is & en-zh & en-ru \\
\hline
\multicolumn{11}{c}{\textit{N=100}} \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Easy instances}} \\
ALMA-\scriptsize{BLEU} & 31.38 & 45.79 & 38.14 & 25.64 & 41.25 & 32.09 & 31.95 & 27.57 & 40.05 & 29.37 \\
Ours-\scriptsize{BLEU} & 32.50 & 46.32 & 40.13 & 25.23 & 40.80 & 31.22 & 31.55 & 26.00 & 39.55 & 29.01 \\
ALMA-\scriptsize{COMET} & 85.57 & 87.71 & 87.82 & 81.38 & 86.26 & 86.84 & 90.90 & 87.61 & 87.14 & 88.80 \\
Ours-\scriptsize{COMET} & 85.50 & 87.67 & 87.71 & 81.24 & 86.17 & 86.02 & 89.84 & 85.80 & 86.39 & 87.89 \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Hard instances}} \\
ALMA-\scriptsize{BLEU} & 12.25 & 29.49 & 21.72 & 1.95 & 15.73 & 15.71 & 12.79 & 17.51 & 14.59 & 15.45 \\
Ours-\scriptsize{BLEU} & 15.56 & 35.93 & 27.72 & 4.62 & 19.77 & 16.15 & 16.67 & 17.13 & 19.49 & 15.54 \\
ALMA-\scriptsize{COMET} & 62.73 & 67.08 & 72.62 & 49.94 & 62.64 & 58.50 & 60.80 & 70.02 & 59.07 & 62.31 \\
Ours-\scriptsize{COMET} & 65.98 & 71.16 & 75.12 & 58.99 & 67.19 & 60.90 & 67.90 & 71.57 & 62.03 & 65.16 \\
\hline
\multicolumn{11}{c}{\textit{N=200}} \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Easy instances}} \\
ALMA-\scriptsize{BLEU} & 31.96 & 47.11 & 39.94 & 26.22 & 42.13 & 32.5 & 32.75 & 28.54 & 41.08 & 30.22 \\
Ours-\scriptsize{BLEU} & 33.10 & 47.41 & 41.60 & 25.79 & 41.43 & 31.52 & 32.20 & 26.91 & 40.48 & 29.79 \\
ALMA-\scriptsize{COMET} & 86.34 & 88.61 & 88.72 & 82.31 & 87.02 & 87.76 & 91.85 & 88.67 & 87.97 & 89.67 \\
Ours-\scriptsize{COMET} & 86.16 & 88.40 & 88.43 & 81.98 & 86.89 & 86.75 & 90.77 & 86.94 & 87.12 & 88.73 \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Hard instances}} \\
ALMA-\scriptsize{BLEU} & 17.46 & 30.39 & 24.17 & 6.00 & 20.03 & 19.11 & 14.83 & 19.02 & 18.61 & 15.43 \\
Ours-\scriptsize{BLEU} & 19.31 & 35.04 & 29.25 & 7.55 & 23.70 & 19.96 & 18.16 & 18.29 & 21.52 & 15.95 \\
ALMA-\scriptsize{COMET} & 67.24 & 71.82 & 76.62 & 57.84 & 67.59 & 64.30 & 67.13 & 74.56 & 65.46 & 67.59 \\
Ours-\scriptsize{COMET} & 69.85 & 74.82 & 78.52 & 63.87 & 70.22 & 66.77 & 70.37 & 74.13 & 67.50 & 68.78 \\
\hline
\multicolumn{11}{c}{\textit{N=500}} \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Easy instances}} \\
ALMA-\scriptsize{BLEU}& 34.36 & 50.81 & 46.92 & 28.50 & 45.16 & 34.61 & 35.28 & 31.79 & 43.91 & 32.13 \\
Ours-\scriptsize{BLEU} & 35.33 & 50.59 & 47.25 & 27.82 & 44.16 & 33.25 & 34.07 & 30.00 & 42.92 & 31.67 \\
ALMA-\scriptsize{COMET} & 88.08 & 90.54 & 91.04 & 84.29 & 88.62 & 89.59 & 93.66 & 91.08 & 89.79 & 91.47 \\
Ours-\scriptsize{COMET} & 87.80 & 90.10 & 90.50 & 83.86 & 88.40 & 88.55 & 92.48 & 89.57 & 88.79 & 90.61 \\
\cline{2-11}
\multicolumn{11}{c}{\textit{Hard instances}} \\
ALMA-\scriptsize{BLEU} & 21.31 & 35.46 & 28.66 & 13.08 & 25.4 & 22.53 & 19.82 & 22.52 & 24.81 & 19.78 \\
Ours-\scriptsize{BLEU} & 23.09 & 37.91 & 32.66 & 14.04 & 27.32 & 22.89 & 22.38 & 21.32 & 26.58 & 19.78 \\
ALMA-\scriptsize{COMET} & 73.56 & 78.24 & 81.55 & 67.07 & 74.39 & 72.74 & 76.38 & 80.61 & 73.38 & 75.29 \\
Ours-\scriptsize{COMET} & 74.77 & 79.75 & 82.41 & 69.56 & 75.63 & 73.24 & 77.34 & 79.19 & 74.12 & 74.97 \\
\hline
\multicolumn{11}{c}{\textit{Overall performance, i.e., N=infinite when all instances are included.}} \\
ALMA-\scriptsize{BLEU} & 30.73 & 44.68 & 36.46 & 24.15 & 40.37 & 31.37 & 31.12 & 26.67 & 39.05 & 28.76 \\
Ours-\scriptsize{BLEU} & 31.93 & 45.60 & 38.85 & 23.94 & 40.09 & 30.64 & 30.91 & 25.22 & 38.76 & 28.43 \\
ALMA-\scriptsize{COMET} & 84.42 & 86.29 & 86.3 & 79.70 & 85.09 & 85.45 & 89.42 & 85.85 & 85.76 & 87.50 \\
Ours-\scriptsize{COMET} & 84.50 & 86.53 & 86.45 & 80.05 & 85.22 & 84.78 & 88.75 & 84.38 & 85.19 & 86.77 \\
\hline
\end{tabular}
% }
\end{table*}

==> tables/data_stat.tex <==
\begin{table*}
    \centering
    \begin{tabular}{c|c|c|c}
        \hline
        Translation Tool & Translation Direction & \# Training Set & \# Development Set  \\
        \hline
        \multirow{10}{*}{DeepL/Google Translate}& $cs \rightarrow en$ & &  \\\cline{2-4}
                                                   & $en \rightarrow cs$ & & \\\cline{2-4}
                                                   & $de \rightarrow en$ & & \\\cline{2-4}
                                                   & $en \rightarrow de$ & & \\\cline{2-4}
                                                   & $is \rightarrow en^*$ & & \\\cline{2-4}
                                                   & $en \rightarrow is^*$ & & \\\cline{2-4}
                                                   & $zh \rightarrow en$ & & \\\cline{2-4}
                                                   & $en \rightarrow zh$ & & \\\cline{2-4}
                                                   & $ru \rightarrow en$ & & \\\cline{2-4}
                                                   & $en \rightarrow ru$ & & \\\cline{2-4}
        \hline
        \multirow{10}{*}{ChatGPT}& $cs \rightarrow en$ & & \\\cline{2-4}
                                                     & $en \rightarrow cs$ & & \\\cline{2-4}
                                                     & $de \rightarrow en$ & & \\\cline{2-4}
                                                     & $en \rightarrow de$ & & \\\cline{2-4}
                                                     & $is \rightarrow en$ & & \\\cline{2-4}
                                                     & $en \rightarrow is$ & & \\\cline{2-4}
                                                     & $zh \rightarrow en$ & & \\\cline{2-4}
                                                     & $en \rightarrow zh$ & & \\\cline{2-4}
                                                     & $ru \rightarrow en$ & & \\\cline{2-4}
                                                     & $en \rightarrow ru$ & & \\\cline{2-4}
        \hline
        % \multirow{10}{*}{NLLB}   & $cs \rightarrow en$ & & \\\cline{2-4}
        %                                              & $en \rightarrow cs$ & & \\\cline{2-4}
        %                                              & $de \rightarrow en$ & & \\\cline{2-4}
        %                                              & $en \rightarrow de$ & & \\\cline{2-4}
        %                                              & $is \rightarrow en$ & & \\\cline{2-4}
        %                                              & $en \rightarrow is$ & & \\\cline{2-4}
        %                                              & $zh \rightarrow en$ & & \\\cline{2-4}
        %                                              & $en \rightarrow zh$ & & \\\cline{2-4}
        %                                              & $ru \rightarrow en$ & & \\\cline{2-4}
        %                                              & $en \rightarrow ru$ & & \\\cline{2-4}
        % \hline
        \multirow{10}{*}{Human} & $cs \rightarrow en$ & & \\\cline{2-4}
                                                    & $en \rightarrow cs$ & & \\\cline{2-4}
                                                    & $de \rightarrow en$ & & \\\cline{2-4}
                                                    & $en \rightarrow de$ & & \\\cline{2-4}
                                                    & $is \rightarrow en$ & & \\\cline{2-4}
                                                    & $en \rightarrow is$ & & \\\cline{2-4}
                                                    & $zh \rightarrow en$ & & \\\cline{2-4}
                                                    & $en \rightarrow zh$ & & \\\cline{2-4}
                                                    & $ru \rightarrow en$ & & \\\cline{2-4}
                                                    & $en \rightarrow ru$ & & \\\cline{2-4}
        \hline
        
    \end{tabular}
    \caption{The statistics of our data. $*$: Icelandic ($is$) is not supported by the DeepL API; therefore, we utilize the Google Translate API as an alternative.}
    \label{tab:statistics_data}
\end{table*}
